Zero-Shot Metric Depth Estimation via Monocular Visual-Inertial Rescaling for Autonomous Aerial Navigation

This paper presents a methodology to predict metric depth from monocular RGB images and an inertial measurement unit (IMU). To enable collision avoidance during autonomous flight, prior works either leverage heavy sensors (e.g., LiDARs or stereo cameras) or data-intensive and domain-specific fine-tuning of monocular metric depth estimation methods. In contrast, we propose several lightweight zero-shot rescaling strategies to obtain metric depth from relative depth estimates via the sparse 3D feature map created using a visual-inertial navigation system. These strategies are compared for their accuracy in diverse simulation environments. The best performing approach, which leverages monotonic spline fitting, is deployed in the real-world on a compute-constrained quadrotor. We obtain on-board metric depth estimates at 15 Hz and demonstrate successful collision avoidance after integrating the proposed method with a motion primitives-based planner.

==> preamble.tex <==
% to typeset URLs, URIs, and DOIs
\usepackage{url}
\def\UrlFont{\rmfamily}

% link youtube videos
\usepackage[bookmarks=true]{hyperref}

% reduce figure caption size
\usepackage{caption}

\usepackage[square,sort&compress,comma,numbers]{natbib}

\usepackage{array}
\usepackage{float}
\usepackage[capitalise]{cleveref}
\usepackage[binary-units=true]{siunitx}
\sisetup{per-mode=symbol,detect-weight=true}
\usepackage{subfig}
\usepackage{balance}

\usepackage{xcolor}
\usepackage{booktabs}

% Loads tikz plots
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\pgfplotsset{compat=1.16}

\usepackage{tikz}
% Load the library
\usetikzlibrary{external,positioning}
% Enable the library !!!>>> MUST be in the preamble <<<!!!!
\usepgfplotslibrary{external}
\tikzexternalize[prefix=tikzext/]

% Import Sarah Furnace Map
\usepackage{pdfpages}
\RequirePackage{luatex85}
\def\pgfsysdriver{pgfsys-pdftex.def}

% https://tex.stackexchange.com/questions/57484/is-there-a-way-to-control-whitespace-around-a-tikz-picture
\usepackage{adjustbox}

% Manage ArXiv submissions
\usepackage{ifthen}
% Enable this for arxivmode
\newcommand\arxivmode{true}
\ifthenelse{\equal{\arxivmode}{true}}{\pdfoutput=1}{}

\usepackage{graphics} % for pdf, bitmapped graphics files
\usepackage{graphicx}
\DeclareGraphicsExtensions{.pdf,.png,.jpg}

\usepackage{epsfig} % for postscript graphics files

\usepackage{amsmath} % assumes amsmath package installed

%\let\Bbbk\relax
%\usepackage{amssymb}  % assumes amsmath package installed
\usepackage{balance} % for references

\newcommand{\round}[1]{\ensuremath{\lfloor#1\rceil}}


% To display all fbox'es around figures, set \vizfbox{true}
% To remove all fbox'es around figures set \vizfbox{false}
\newcommand\vizfbox{true}
\newcommand\vizbox[2]{\ifthenelse{\equal{#1}{false}}{\fbox{#2}}{#2}}

\definecolor{green}{RGB}{0,146,0}
\newcommand{\red}[1]{{\color{red}{#1}}}
\newcommand{\blue}[1]{{\color{blue}{#1}}}
\newcommand{\green}[1]{{\color{green}{#1}}}

\usepackage[font=small]{caption} % Make caption size small instead of normal

\usepackage{graphicx} % Required for images
\graphicspath{{imgs/}} % Folder where images are stored
